DLA: Compiler and FPGA Overlay for Neural Network Inference Acceleration

Overlays have shown significant promise for field-programmable gate-arrays (FPGAs) as they allow for fast development cycles and remove many of the challenges of the traditional FPGA hardware design flow. However, this often comes with a significant performance burden resulting in very little adoption of overlays for practical applications. In this paper, we tailor an overlay to a specific application domain, and we show how we maintain its full programmability without paying for the performance overhead traditionally associated with overlays. Specifically, we introduce an overlay targeted for deep neural network inference with only ~1% overhead to support the control and reprogramming logic using a lightweight very-long instruction word (VLIW) network. Additionally, we implement a sophisticated domain specific graph compiler that compiles deep learning languages such as Caffe or Tensorflow to easily target our overlay. We show how our graph compiler performs architecture-driven software optimizations to significantly boost performance of both convolutional and recurrent neural networks (CNNs/RNNs) - we demonstrate a 3x improvement on ResNet-101 and a 12x improvement for long short-term memory (LSTM) cells, compared to naive implementations. Finally, we describe how we can tailor our hardware overlay, and use our graph compiler to achieve ~900 fps on GoogLeNet on an Intel Arria 10 1150 - the fastest ever reported on comparable FPGAs.

==> folding.tex <==
\hl{Author: David Han}

%-----------------------------------------------------------------------------

While DLA dedicates most of the compute resources to perform convolutions
efficiently, it adapts well to non-convolution primitives by mapping most of
them to convolutions.
%
The rationale is that, when these primitives occur {\em infrequently} in the
network, any resources dedicated to them are under-utilized (over time),
leading to lower overall efficiency compared to reusing the existing powerful
convolution engine.
%
This section describes the mapping of three primitives to convolution:
%
\begin{itemize}
\item Fully-connected layer
\item Average pooling
\item Element-wise addition
\end{itemize}

%-----------------------------------------------------------------------------

\subsection{Fully-Connected (FC) Layer}

An FC layer effectively performs a multiplication between a vector (input)
and a matrix (weights).
%
It can be mapped to a convolution as follows:
%
1) the 1D FC input of length $N$ is mapped to a 3D convolution input of shape
   $1 \times 1 \times N$, and
%
2) the 2D FC weight matrix of shape $N \times M$ is mapped to $M$ 3D
   convolution filters of shape $1 \times 1 \times N$.
%
With this mapping, the computation of each FC output is assigned to a PE.

%-----------------------------------------------------------------------------

\subsection{Average Pooling}

Average pooling of window $H \times W$ on a 2D image is equivalent to a 2D
convolution with a filter of size $H \times W$.
%
Each filter element is of value $1 / (H \times W)$.
%
We call this filter a {\em average pooling filter}.
%
For a 3D input of depth $D$, average pooling is applied to {\em each} 2D input
surface, producing the corresponding output surface.
%
In this case, the equivalent convolution filter for the output surface at
depth $d$, is of shape $H \times W \times D$, with all zero filter values
except the surface at depth $d$ being the average pooling filter.
%
[EDIT: add a diagram here]

%-----------------------------------------------------------------------------

\subsection{Element-wise Addition}

Figure~\ref{fig:eltwise-conv} illustrates the mapping of element-wise addition
of two 3D inputs ($IN_1$ and $IN_2$) to a convolution.
%
Assuming both inputs are of shape $H \times W \times D$, we first concatenate
them depth-wise, forming a merged input $IN$ of shape $H \times W \times 2D$.
%
Then we apply a convolution to $IN$ with $D$ filters of shape $1 \times 1
\times 2D$.
%
Each filter is effectively responsible for (element-wise) summing two
corresponding surfaces in $IN_1$ and $IN_2$.
%
Therefore, all filter values are 0 except two 1's at the corresponding
surfaces' depths.
%

%---------------------------------------

\begin{figure*}[ht]
\centering
\subfigure[Convolution on a single depth-concatenated input.]{
% \includegraphs[width=0.8\linewidth]{tbf.pdf}
}
\quad
\subfigure[Convolution filter values.]{
% \includegraphs[width=0.8\linewidth]{tbf.pdf}
}
\caption{Mapping of element-wise addition
of two 3D inputs ($IN_1$ and $IN_2$) to a convolution.}
\label{fig:eltwise-conv}
\end{figure*}

%---------------------------------------

\subsection{Sparse Filter Optimization}

A convolution filter is considered {\em sparse} when most of its values are
zeros.
%
In such cases, we can eliminate the filter data fetch and the computation
corresponding to the zero entries.
%
[EDIT: elaborate]

%-----------------------------------------------------------------------------

\subsection{}

%-----------------------------------------------------------------------------

\section{Layer Merging Optimizations}
\hl{mohamed: I think this should be called Resnet-specific optimizations -- it's good to go in detail about optimizing a well-defined workload, then mention the generality of the optimization on the NN pattern.}
This should be a separate section -- not sub-section.

\begin{itemize}
\item Conv + eltwise merging
\item FC merging -- establish FC-conv equivalency
\end{itemize}

